SUVR: A Search-based Approach to Unsupervised Visual Representation Learning

Unsupervised learning has grown in popularity because of the difficulty of collecting annotated data and the development of modern frameworks that allow us to learn from unlabeled data. Existing studies, however, either disregard variations at different levels of similarity or only consider negative samples from one batch. We argue that image pairs should have varying degrees of similarity, and the negative samples should be allowed to be drawn from the entire dataset. In this work, we propose Search-based Unsupervised Visual Representation Learning (SUVR) to learn better image representations in an unsupervised manner. We first construct a graph from the image dataset by the similarity between images, and adopt the concept of graph traversal to explore positive samples. In the meantime, we make sure that negative samples can be drawn from the full dataset. Quantitative experiments on five benchmark image classification datasets demonstrate that SUVR can significantly outperform strong competing methods on unsupervised embedding learning. Qualitative experiments also show that SUVR can produce better representations in which similar images are clustered closer together than unrelated images in the latent space.

==> Content/2-relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}
\textbf{Self-supervised learning.}
The way to overcome the problem data without labels is using inherent information of data as ground-truth for training. Specifically, we can split an image to different context segments \cite{doersch2015unsupervised} then use the relative position as supervised information for embedding learning. Besides, data augmentation is frequently be used in self-supervised learning because it can make embedding more robust compare to non-augmented \cite{wang2017effectiveness}. For example, we can do the different combinations of rotate, resize and random crop to one image then discriminate the image from different augmentation. Recently, a novelty criterion called contrastive loss \cite{chen2020simple} has proposed, they compare the different and identical parts between the image pairs of augmentation for embedding learning. \\

\noindent
\textbf{Generative model.}
Unsupervised learning tries to learn the distribution of data itself. In particular, Auto-encoder \cite{autoencoder} learns the embedding through mapping the image to the low dimension hidden state then minimizing the reconstruct loss between the original image. 
On the other hand, Generative adversarial networks \cite{radford2015unsupervised} \cite{goodfellow2014generative} train the embedding of the bottleneck by the min-max game that
minimize the probability of discriminating the generated image from normal distribution as true, hence has a better ability for embedding learning. \\

% \textbf{Feature based approach.}
% These approaches consider the relations within the batch \cite{li2014efficient} for embedding learning. In particular, utilizing two different augmentations on one image can generate two images, then SimCLR \cite{chen2020simple} discriminate these two images whether they belong to the same image, hence they consider the relationship between the image pairs. However, ISIF \cite{Ye_2019} further separates the other embedding of augmented images in the same batch. The difference between them is the ISIF forcing the embedding to separate from different images in batch, then the embedding will be more discriminating \cite{azulay2018deep} than the SimCLR.

\noindent
\textbf{Memory based approach.}
Comparing to only consider instances in batch, the memory-based approach further discuss the relation between batch and the whole image set. It will cause the model to have more information for embedding learning in unsupervised settings. Specifically, Lemniscate \cite{wu2018unsupervised} utilizes the relation between an instance and the whole image set to do instance-wise discrimination. Additionally, AND \cite{huang2019unsupervised} further consider the relation by the similarity that adaptively choosing the anchor-neighborhood to close the embedding of those instances.

\begin{table}[!th]
    \centering
    \caption{Comparison of the related work.}
    \label{tab:comparision} 
    \centering
     \begin{tabular}{ccccc} 
     \bottomrule
      & Close & Separate & Relation & Explore\\
     \toprule
     Lemniscate & - & \checkmark & \checkmark & -\\ 
     ISIF & \checkmark & \checkmark & - & -\\
     SimCLR & \checkmark & - & - & -\\ 
     AND & \checkmark & - & \checkmark & -\\ 
     \hline
     SUVR & \checkmark & \checkmark & \checkmark & \checkmark\\
     \toprule
    \end{tabular}
\end{table}

Existed work considers the different approaches to do unsupervised embedding learning respectively. On Table\ref{tab:comparision}, the column of "close" means whether update the embedding by closing the similar instances; "separate" represents whether use the dissimilar instance as auxiliary information to update the embedding; "relation" imply whether use memory to consider the complex relationship between instances for updating the embedding; "explore" represent whether the model has the ability to explore meaningful instances. It's worth noticing that consider exploitation and exploration simultaneously are important for embedding learning. Our proposed NB-DSCV not only makes the embedding closing to similar and separating from dissimilar instances but also have the ability to explore different neighbors for curriculum learning, and enhance the performance of unsupervised embedding learning task.

==> Content/3-problem.tex <==
\section{Problem Definition}
\label{sec:problemdefinition}
Given a set of $n$ images without annotation $\mathcal{D} =  \{\mathbf{x}_1, \mathbf{x}_2, ..., \mathbf{x}_n\}$, we learn a function $\mathcal{F}_\theta$ which maps $\mathbf{x}$ to representative embeddings $\mathbf{v}$, i.e., $\mathbf{v} = \mathcal{F}_\theta (\mathbf{x})$. The representative embeddings $\mathbf{v}$ should have closer distance between similar images while being seperated from dissimilar instances.
Specifically, we propose using BFS and DFS to discover neighbors. Among the explored neighbor, we denote positive neighbors as $N_{pos}$ for each instance, and negative neighbors as $N_{neg}$. We iteratively conduct neighbor search, and reset the found neighbors for each iteration in a curriculum learning manner.
% as auxiliary information for embedding update. Additionally, we reset the neighbors for each round $R$ to consider more information in curriculum learning. In the following section, we will discuss each component of NB-DSCV in detail.
